Eight Years of Face Recognition Research: Reproducibility, Achievements and Open Issues

Automatic face recognition is a research area with high popularity. Many different face recognition algorithms have been proposed in the last thirty years of intensive research in the field. With the popularity of deep learning and its capability to solve a huge variety of different problems, face recognition researchers have concentrated effort on creating better models under this paradigm. From the year 2015, state-of-the-art face recognition has been rooted in deep learning models. Despite the availability of large-scale and diverse datasets for evaluating the performance of face recognition algorithms, many of the modern datasets just combine different factors that influence face recognition, such as face pose, occlusion, illumination, facial expression and image quality. When algorithms produce errors on these datasets, it is not clear which of the factors has caused this error and, hence, there is no guidance in which direction more research is required. This work is a followup from our previous works developed in 2014 and eventually published in 2016, showing the impact of various facial aspects on face recognition algorithms. By comparing the current state-of-the-art with the best systems from the past, we demonstrate that faces under strong occlusions, some types of illumination, and strong expressions are problems mastered by deep learning algorithms, whereas recognition with low-resolution images, extreme pose variations, and open-set recognition is still an open problem. To show this, we run a sequence of experiments using six different datasets and five different face recognition algorithms in an open-source and reproducible manner. We provide the source code to run all of our experiments, which is easily extensible so that utilizing your own deep network in our evaluation is just a few minutes away.

==> biography.tex <==
% if you will not have a photo at all:


\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/phototiago.jpg}}]{Tiago de Freitas Pereira}
   received the Ph.D. degree in Electrical Engineering from Ecole Polytechnique Federale de Lausanne ( http://www.epfl.ch) in Switzerland (2019) whose main contribution was the development of the Domain Specific Units (DSU) framework for Heterogeneous Face Recognition.
   Currently, he is a research associate at the Idiap Research Institute in the Biometrics Security and Privacy group and conducts research on face recognition.
   \end{IEEEbiography}
   
   
   %\vspace{-2em}
   %\vspace{-50em}


   
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/dominic.jpeg}}]{Dominic Schmidli}
    received the B.S. degree on Computer Science from the University of Zurich (http://www.uzh.ch) in Switzerland (2019), where he conducted
    research on automatic Face Recognition.
\end{IEEEbiography}
    

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/photolinghu.png}}]{Yu Linghu} 
    received the B.S. degree in Mathematics from The Ohio State University (US) in 2019, and Master's Degree in Data Science from the University of Zurich in 2022. 
    Currently, she is a Ph.D. student supervised by Prof. Dr. Manuel G\"unther in the Artificial Intelligence and Machine Learning Group at the Department of Informatics of the University of Zurich. 
    Her research focuses on investigating fairness aspects in Face Recognition (Biometrics) models, which is part of a collaboration project with the Idiap Research Institute.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/photozhang.png}}]{Xinyi Zhang}
    is a Ph.D. student from March 2022 at the University of Zurich in the Artificial Intelligence and Machine Learning group, supervised by Prof. Dr. Manuel G\"unther. 
    She received Bachelor’s diploma major in Computer Science and Technology from the University of Zhengzhou (China). And she got a Master\'s degree from the University of Zurich Data Science. 
    From 2021, she started to focus on biometrics recognition especially face recognition. Now her research is to improve face recognition performance in low-resolution datasets.
\end{IEEEbiography}



\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/photosebastien.png}}]{S{\'e}bastien Marcel}
   is the head of the Biometrics group and senior research scientist at the Idiap Research Institute (CH), where he leads a research team and conducts research on biometrics and more particularly face recognition, speaker recognition, vein recognition and spoofing/anti-spoofing.
   He received the Ph.D. degree in signal processing from Universit{\'e} de Rennes I in France (2000) at CNET, the research center of France Telecom (now Orange Labs).
   He is currently interested in pattern recognition and machine learning with a focus on multimodal biometric person recognition.
   
\end{IEEEbiography}
   

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pictures/Manuel_Guenther.png}}]{Manuel G\"unther} is an assistant Professor for Artificial Intelligence
     and Machine Learning at the Department of Informatics of the University of Zurich, where he conducts research on the classification of samples under the presence of unknown classes 
     and on automatic face recognition systems.
    He received his doctoral degree (Dr.-Ing.) from the Technical University of Ilmenau in 2012.
    His research interests also include deep learning in general and the phenomenon of adversarial samples in particular.     
\end{IEEEbiography}
    







==> space.tex <==
\usepackage{microtype} 


\makeatletter

\setlength\belowcaptionskip{6pt \@plus 4pt \@minus -6pt}
\setlength\abovecaptionskip{2pt}

% \long\def\@makecaption#1#2{
% \vspace*{\abovecaptionskip}
%    \setbox\@tempboxa\hbox{\small \noindent {\bf #1.}~{\it #2}}
%    \setlength{\@ctmp}{\hsize}
%    \addtolength{\@ctmp}{-\@figindent}\addtolength{\@ctmp}{-\@figindent}
%    % IF longer than one indented paragraph line
%    \ifdim \wd\@tempboxa >\@ctmp
%       % THEN DON'T set as an indented paragraph
%       {\small{\bf #1.}{~\it#2}\par}
%    \else
%       % ELSE center
%       \hbox to\hsize{\hfil\box\@tempboxa\hfil}
%   \fi\vspace*{\belowcaptionskip}}

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-1.2ex \@plus -2ex \@minus -.2ex}%
                                   {.5ex \@plus.2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-.6ex \@plus -2ex \@minus -.2ex}%
                                   {.5ex \@plus.2ex}%
	                           {\normalfont\large\bfseries}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-.5ex\@plus -.2ex \@minus -.2ex}%
                                     {.2ex \@plus .2ex}%
                                     {\normalfont\large\bfseries}}

\abovedisplayskip=1pt plus 3pt minus 6pt 
\abovedisplayshortskip=0pt plus 3pt 
\belowdisplayskip=1pt plus 3pt minus 6pt 
\belowdisplayshortskip=0pt plus 3pt minus 3pt 

\floatsep 4pt plus 2pt minus 2pt 
\textfloatsep 4pt plus 2pt minus 4pt
\intextsep 2pt plus 2pt minus 2pt  
\dblfloatsep 4pt plus 2pt minus 2pt 
\dbltextfloatsep 6pt plus 2pt minus 4pt 
\@fptop 2pt plus 1fil \@fpsep 6pt plus 2fil \@fpbot 0pt plus 1fil 
\@dblfptop 6pt plus 1fil \@dblfpsep 6pt plus 2fil \@dblfpbot 2pt plus 1fil


\makeatother

\def\closemath{
\abovedisplayskip=3pt plus 3pt minus 1pt 
\abovedisplayshortskip=0pt plus 1pt minus 1pt 
\belowdisplayskip=3pt plus 3pt minus 1pt 
\belowdisplayshortskip=0pt plus 1pt minus 1pt }

\def\tightmath{
\abovedisplayskip=4pt plus 2pt minus 1pt 
\abovedisplayshortskip=2pt plus 1pt minus 1pt 
\belowdisplayskip=4pt plus 2pt minus 1pt 
\belowdisplayshortskip=2pt plus 1pt minus 1pt }
\def\crushmath{
\abovedisplayskip=1pt plus 1pt minus 2pt 
\abovedisplayshortskip=1pt plus 1pt minus 2pt 
\belowdisplayskip=1pt plus 1pt minus 2pt 
\belowdisplayshortskip=1pt plus 1pt minus 2pt }
\tightmath

